Collaborative Anomaly Detection

In recommendation systems, items are likely to be exposed to various users and we would like to learn about the familiarity of a new user with an existing item. This can be formulated as an anomaly detection (AD) problem distinguishing between "common users" (nominal) and "fresh users" (anomalous). Considering the sheer volume of items and the sparsity of user-item paired data, independently applying conventional single-task detection methods on each item quickly becomes difficult, while correlations between items are ignored. To address this multi-task anomaly detection problem, we propose collaborative anomaly detection (CAD) to jointly learn all tasks with an embedding encoding correlations among tasks. We explore CAD with conditional density estimation and conditional likelihood ratio estimation. We found that: $i$) estimating a likelihood ratio enjoys more efficient learning and yields better results than density estimation. $ii$) It is beneficial to select a small number of tasks in advance to learn a task embedding model, and then use it to warm-start all task embeddings. Consequently, these embeddings can capture correlations between tasks and generalize to new correlated tasks.

==> coldstart.tex <==
\section{Item Embeddings Initialization}\label{sec:init_embeddings}
Using random initialization for CTR models is typically not the best choice in practice.
\rh{why?}
In this section, we focus on \textit{learning} a tailored item embedding \(\widehat{\vv}_m\) that can be used in initialization of (\ref{eq:ctr}), given the pre-embedding model on impression data.
We seek item embeddings with the following properties:
%
\begin{enumerate}
    \item (\textbf{Correlation}) Similar to~\cite{meyerson2020traveling}, we find that randomly initialized item embeddings do not fully exploit item similarities during training, even with fine-tuning.
    To overcome this, the learned initialization should capture item similarity.
    \item (\textbf{Generalization}) The learned item embedding models can generalize to cold start items and new items which are absent when training the pre-embedding model.
    \item (\textbf{Efficiency}) Since each item \(m\) can be identified as a distribution \(q_m(\uv)\),
    a natural measurement of item similarity is to calculate their distributional distances.
    However, this requires an enormous number of samples to approximate all pair-wise distances.
    By contrast, the acquisition of learned item embeddings should be inexpensive.
    % \item (\textbf{Interpretability}
\end{enumerate}

% \subsection{Training procedure}

Suppose there are \(M\) items in total, in which $|\mathcal{V}^w|$ are warm start items that has at least \(T\) user clicks.
We propose to learn the item embedding \(\widehat{\vv}_m\) by first training a \emph{pre-embedding model} on warm start items, and then use the pre-embedding model to encode all items.
% selecting \(M_0\ll M\) \emph{seed items} from the warm start items to train a \emph{pre-embedding model}, and then use the pre-embedding model to encode all items.
In practice, we find that randomly selecting \(M_0\ll |\mathcal{V}^w|\) \emph{seed items} from the warm start items are representative enough to capture correlations among all items.
This is the case, presumably, due to the redundancy among items where the inherent complexity of semantics may not be that big.
We study the choice of \(M_0\) in Section~\ref{sec:exp}.

\subsection{Train pre-embedding model with seed items}
Without loss of generality, seed items are identified as item \(1\) to \(M_0\).
We train a log-likelihood ratio task to get the pre-embedding model by calling \(\psi,\ev=\textproc{EstimateCLR}(M_0)\) in Algorithm~\ref{alg:mtocc}, where \(\psi\) denotes the parameters of the pre-embedding model (not related to the final CTR model).
The returned vector \(\ev=\ev_1,\ldots,\ev_{M_0}\) and the pre-embedding model \(\psi\) is sent to the next step.

\subsection{Obtaining task embeddings initializations}
Given the pre-embedding model \(\psi\), the following basis functions are constructed,
\begin{equation}\label{eq:response_vec}
    \vr(\uv)=\left(\vr_1(\uv), \ldots, \vr_{M_0}(\uv)\right),\nonumber
\end{equation}
where \(\vr_m(\uv)=\log(q_m(\uv)/p(\uv))\) is the log-likelihood ratio of the pre-embedding model \(\psi\).
The item embedding \(\widehat{\vv}_m\) is defined as a linear projection of \(q_m(\uv)\) onto these basis functions, \ie,
\begin{align}\label{eq:moh_embeeding_vec}
\widehat{\vv}_m = \left(\mathbb{E}_{q_m(\uv)}[\vr_1(\uv)],\ldots, \mathbb{E}_{q_m(\uv)}[\vr_{M_0}(\uv)]\right).
\end{align}
We independently draw \(N_m\) samples \(\uv_1,\ldots,\uv_{N_m}\) from \(q_m(\uv)\) to estimate \(\widehat{\vv}_m\), where each entry is estimated by \(\mathbb{E}_{q_m(\uv)}[\vr_{m^\prime}(\uv)]\approx\frac{1}{N_m}\sum_{n=1}^{N_m} f(\uv_n,\ev_{m^\prime},\psi)\).
This step only requires forward passing and does not involve any model updates.

After obtaining the learned item embedding initializations \(\widehat{\vv}=(\widehat{\vv}_1,\ldots,\widehat{\vv}_M)\), we can run the CTR model.
This completes the algorithm.

\subsection{Interpreting learned embeddings}

To informally explain why the item embedding initialization \(\widehat{\vv}_m\) in~(\ref{eq:moh_embeeding_vec}) captures item correlations, we treat \(q_m(\vu)\) and \(r_{m^\prime}(\uv)\) as infinite-dimensional vectors by varying \(\uv\) across its support.
Random-projection theory guarantees that \(\text{sim}(\widehat{\vv}_m,\widehat{\vv}_{m^\prime})\approx\text{sim}(q_m,q_{m^\prime})\), when \(M_0\rightarrow\infty\) with random regular basis functions \(\vr(\uv)\) and properly chosen similarity metrics~\cite{gottlieb2015nonlinear}.
In practice, naively generated random functions may not work well, since the random function must capture the difference of \(q_m\) and \(q_{m^\prime}\) on their support.
Likelihood ratios are more reasonable to cover all supports, while still being discriminative since they are learned by contrastive pairs on the population support \(\text{supp}(p(\uv))\).
In our experiments, we found the number of basis functions \(M_0\) can be much smaller than the total number of items \(M\) when tasks are correlated and redundant.
As we will show in experiments, the learned embedding can also generalize to even previously unseen items.


==> experiment_likelihood_ratio.tex <==
\section{conditional likelihood ratio estimation}

We start with experiments on the MovieLens 1M dataset to demonstrate that \(i\)) CAD with conditional likelihood ratio estimation achieves much better results compared to conditional density estimation; and \(ii\)) task embedding initialization is crucial.
To further analyze these properties, we design a set of experiments on an image dataset (CIFAR10) with synthesized tasks.
Unless otherwise stated, all experiments are executed on a single NVIDIA Titan Xp GPU with 12,196M Memory.

\subsection{Experiments on MovieLens 1M}\label{subsec:movielens}

\paragraph{Problem setup}
The MovieLens 1M dataset contains approximately \(3,900\) movies and \(6,040\) users, together with over one million ratings~\cite{harper2015movielens},
hence \(3,900\) AD tasks in total, one for each movie.
We ignore all rating scores and only keep the binary information of whether movies are rated (exposed) or not.
We split users into training and testing sets with 8:2 ratio.
The goal for each AD task is to distinguish between ``common users'' (nominal) and ``fresh users'' (anomalous) in the testing set.

\paragraph{Feature pre-processing}
In MovieLens 1M data, there are four categorical labels for users: gender \((u_g)\), age \((u_a)\), occupation \((u_o)\), and zip-code \((u_z)\); and three categorical features for items: movie id, title, and genre.
We use a deep factorization-machine~\cite{guo2017deepfm} to extract user embeddings \(\xv\) (details in appendix) for training AD models.
The detailed four categorical labels \(u_{n,g},\;u_{n,a},\;u_{n,o},\;u_{n,z}\) for user \(\xv_n\) will be used for testing only.

\paragraph{Nominal and anomalous}
The definition of anomalous varies across domains~\cite{ruff2021unifying}.
We consider point anomaly in the context of recommendation systems, which aims to identify each anomalous user for an item \(t\).
An anomalous user is defined according to a specific user label.
Take the label ``age'' as an example.
Suppose an item \(t\) is exposed to a set of users \(\Xv^{(t)}=\{\xv^{(t)}_1,\ldots,\xv^{(t)}_{m^{(t)}}\}\), where the age of user \(\xv^{(t)}_n\) is \(u^{(t)}_{n,a}\). We identify the most frequent age category \(\hat{u}^{t}_a:=\arg\max_u \sum_{n=1}^{m^{(t)}}\mathbf{1}(u_{n,a}^{(t)}=u)\) as nominal and the least frequent age category \(\check{u}^{t}_a:=\arg\min_u \sum_{n=1}^{m^{(t)}}\mathbf{1}(u_{n,a}^{(t)}=u)\) as anomalous.
The AUC score is calculated on the test set by distinguishing between the nominal and anomalous users only.
Since there are multiple user labels, we may report multiple AUC scores, one for each user label.
In our experiments below, we test on two user labels: ``Age'' with 5 binned categories and ``Occupation'' with 21 categories.

\paragraph{Task filtering}
We remove tasks that are not eligible for AD experiments.
To be precise, we first remove tasks with fewer than 100 exposures.
Among the remaining tasks, we select \(50\%\) of them with the lowest user label histogram entropy, indicating nominal and anomalous are distinguishable.
There are 1,629 remaining tasks after the filtering.

\paragraph{Methods}
We study CAD with the proposed conditional likelihood ratio estimation method and two conditional density estimation methods, conditional Gaussian and conditional normalizing flows.
For conditional likelihood ratio estimation, we implement a 3-layer MLP, where task embeddings are concatenated to the input.
For Gaussian, we use a 3-layer MLP with two output heads to map the task embedding to Gaussian mean and variance.
For normalizing flows, we follow~\cite{papamakarios2017masked} to stack \(5\) blocks,
where each block is a stack of MADE~\cite{germain2015made} and BatchNorm.
For all methods, we train until their losses do not decrease, and select the best checkpoints on validation and report results on testing data.
Implementation details are put in %\textcolor{red}{Appendix}.
appendix.

The AUC results are shown in Table~\ref{table:movielens} (left).
Conditional density estimation completely fails in the CAD scenario, on both ``Age'' labels and on ``Occupation'' labels.
Normalizing flows are much more flexible than Gaussian, yet still not able to discriminate the anomalous.
This is because density estimation usually requires large data and model capacity for learning.
When conditioning on too many tasks, density estimation may fail to distinguish the complex correlations among tasks.
This phenomenon will be further inspected in Section~\ref{sec:mnist_cifar}.

\paragraph{Task embedding initialization}
In conditional likelihood ratio estimation, task embedding \(\ev^{(t)}\) plays a critical role for data sharing across tasks, since learning one task can enhance the learning of another related task with a similar task embedding.
We compare the following choices of task embedding initialization.
\(i\)) \textit{Graph Embedding}: use learned movie features through a knowledge graph base using KTUP~\cite{cao2019unifying} to initialize \(\ev^{(t)}\).
\(ii\)) \textit{Histogram Embedding}: when training on age labels, we calculate the histogram of users' age labels for each task \(t\): \(\{u^{(t)}_{1,a},\ldots,u^{(t)}_{m^{(t)},a}\}\) to initialize \(\ev^{(t)}\).
This is similarly done for occupations.
\(iii\)) \textit{Random Initialization}: use normal distribution to randomly initialize \(\ev^{(t)}\).
\(iv\)) \textit{Learned Embedding}: initialize \(\ev^{(t)}\) following the procedure in Section~\ref{sec:task_embeddings} with \(M_0=100\) seed tasks. We use the same training scheme for all initialization methods. The training detail can be found in the appendix.


As shown in Table~\ref{table:movielens} (right), task embeddings with additional knowledge (marked with \(*\)) are generally superior over embeddings without such knowledge.
Learned embeddings are significantly better than random embeddings, and even comparable with graph embeddings, since they attempt to uncover the connections underlying over \(1,600\) tasks using seed tasks.

\input{tables/movielens_1m_results}

==> figures/cad_pipeline.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[width=.8\textwidth]{figures/occ_train_proc_v4.pdf}
    \caption{Illustration of the entire training process for $M$ tasks. (a) Sample a subset of $M_0\ll M$ tasks and pre-train the log-likelihood response model as shown in Algorithm~\ref{alg:embed}. (b) For each new task, draw $N^{(t)}$ samples from $q^{(t)}(\xv)$ to estimate the dual embedding $\ev^{(t)}$ following Equation~\ref{eq:moh_embeeding_vec}. (c) Use $\ev^{(t)}$ as task embeddings for MT-OCC\@. The outcome of one step is linked to the next step by dashed lines.}\label{fig:occ_train_proc}
\end{figure*}


==> figures/cifar252.tex <==
\begin{figure*}[t]
%   \begin{center}
  \begin{center}
    % \begin{small}
      \begin{sc}
    \includegraphics[width=\textwidth]{figures/toy_mnist252.pdf}
    % \includegraphics[width=0.2\textwidth]{figures/embeding.pdf}
    \caption{
    }\label{fig:embedding_showcase252}
    \end{sc}
    % \end{small}
  \end{center}
\end{figure*}


==> figures/img_arch_moh.tex <==
% \begin{wrapfigure}[14]{r}{0.5\textwidth}
%     \vspace{-18mm}
\begin{figure}
  \begin{center}
    \includegraphics[width=0.2\textwidth]{figures/moh.pdf}
    \includegraphics[width=0.28\textwidth]{figures/embeding.pdf}
  \end{center}
   \caption{The two multi-task learning framework. The left is the one with multiple output head. The right is embedding based methods. The embedding can be connected or multiplied to any layer of the neural network. Here, we concatenate it with the input data.}
    \label{fig:baseline_framework}
    %\vspace{-3mm}
    \vspace{-3mm}
% \end{wrapfigure}
\end{figure}


==> figures/img_toy_showcase.tex <==
\begin{figure}[!t]
    \centering
    %\begin{subfigure}[c]{0.48\textwidth}
    % \includegraphics[width=0.45\textwidth]{fig/GCKT.pdf}
    %\caption{A}
    %\end{subfigure}
    %\begin{subfigure}%[c]{.48\textwidth}
    \includegraphics[width=0.5\textwidth]{figures/toy_exp.png}
    %\end{subfigure}
    \caption{  
    The novelty defined in this toy example is the category of the digits. These three tasks has different positive set. Different task can own the digit from the same category.}
    \label{fig:wnce_framework}
    %\vspace{-3mm}
    \vspace{-5mm}
\end{figure}



==> figures/img_toy_showcase_mnist.tex <==
% \begin{figure}[!b]
%     \centering
%     %\begin{subfigure}[c]{0.48\textwidth}
%     % \includegraphics[width=0.45\textwidth]{fig/GCKT.pdf}
%     %\caption{A}
%     %\end{subfigure}
%     %\begin{subfigure}%[c]{.48\textwidth}
%     \includegraphics[width=0.5\textwidth]{figures/toy_exp.png}
%     %\end{subfigure}
%     \caption{The novelty defined in this toy example is the category of the digits. These three tasks has different positive set. Different task can own the digit from the same category.}
%     \label{fig:wnce_framework}
%     %\vspace{-3mm}
%     \vspace{-5mm}
% \end{figure}



% \begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}

  \begin{center}
    \includegraphics[width=0.5\textwidth]{figures/toy_exp.png}
  \end{center}
   \caption{
   The novelty in this toy example is defined as the new categories has not been seen. These three tasks have different positive set. Different task can own the digit from the same category.}
    \label{fig:wnce_framework}
    %\vspace{-3mm}
    \vspace{-5mm}
% \end{wrapfigure}
\end{figure}


==> figures/img_toy_showcase_mnist_dist.tex <==
% \begin{wrapfigure}{h}{0.45\textwidth}
\begin{figure}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/toy_example_dist.jpg}
  \end{center}
   \caption{Likelihood estimation of three digits (0,1,2) on three output heads. The difference in distribution on the output heads is large enough for us to distinguish each category.}
    \label{fig:toy_dist}
    %\vspace{-3mm}
    % \vspace{-5mm}
% \end{wrapfigure}
\end{figure}

==> figures/response_dist.tex <==
\begin{figure}[!htb]
%   \begin{center}
  \begin{center}
    % \begin{small}
      \begin{sc}
    % \includegraphics[width=\textwidth]{figures/toy_mnist120.pdf}
            % \subfigure[]{
            \includegraphics[width=0.4\textwidth]{figures/toy_cifar_09_v2.pdf}\vspace{-10pt}
        % \subfigure[]{\label{fig:rep_on_attr}
        % \begin{minipage}{\textwidth}
        %     \includegraphics[width=\textwidth]{figures/toy_cifar_0.png}\\
        %     \includegraphics[width=\textwidth]{figures/toy_cifar_9.png}
        % \end{minipage}
        %         }
        % \subfigure[]{\label{fig:rep_on_attr}
        % }

    % \includegraphics[width=0.2\textwidth]{figures/embeding.pdf}
    % \caption{ Responses
    % }
    \end{sc}
    \caption{ Log-likelihood ratio responses on 120 output heads for two images (airplane and truck) from CIFAR10.
    %digit zero and digit nine on 120 output heads.
    Each output head corresponds to a task containing three out of ten categories in CIFAR10.
    (Left) Orange bars index tasks containing category ``airplane''. (Right) Blue bars index tasks containing category ``truck''. }\label{fig:response_cifar_09}
    % \end{small}
  \end{center}
% \vspace{-2mm}
\end{figure}


==> formulation.tex <==
\section{Problem Formulation}\label{sec:problem}

Given a collection of users \(\mathcal{U}=\{\uv_1,\ldots,\uv_N\}\) and items \(\mathcal{V}=\{\vv_1,\ldots,\vv_M\}\), an event is an interaction between one user and one item. This paper studies two types of binary events: clicks and impressions. In the following, we denote clicks with a $N$-by-$M$ matrix $\mathbf{Y}$, where each entry $y_{nm}\!=\!1$ represents user $n$ clicks item $m$, $y_{nm}\!=\!0$ otherwise. We denote $\mathcal{Y}^+=\{(n,m):y_{nm}=1\}$ as a set of user-item pairs with clicks and $\mathcal{Y}^-=\{(n,m):y_{nm}=0\}$ stands for no-click pairs. When focusing on a single item $m$, we use $\mathcal{Y}^+_m=\{n:y_{nm}=1\}$ to denote the set of users who click item $m$. We use similar notations $z$, $\mathbf{Z}$, and $\mathcal{Z}$ for impressions. Note that a user cannot click on an item without viewing it, thus $\mathcal{Y}^+\subseteq\mathcal{Z}^+$.

The goal of a CTR model is to predict the click probability given user and item embeddings together with context information \(\cv\) (user profile, user's five last clicked items, item targeting, {\em etc}.) as
\begin{align}
p(y_{nm}=1|\uv_n,\vv_m,\cv).
\label{eq:ctr}
\end{align}
We do not assume there is rich context information, as in real scenarios context may be incomplete or missing.
Modern deep CTR models can accurately predict items with abundant user clicks. We denote those as \textit{warm start} items $\mathcal{V}^w=\{m:|\mathcal{Y}_m^+|\geq T_Y, |\mathcal{Z}_m^+|\geq T_Z\}$, where $T_Y$, $T_Z$ is a threshold determined by domain knowledge. In real scenarios, user clicks are sparse for most items. The extreme case consists of \textit{cold start} items $\mathcal{V}^c=\{m:|\mathcal{Y}_m^+|=0, |\mathcal{Z}_m^+| = 0 \}$, for which item embeddings \(\vv_m\) are hard to learn. This paper focuses on improving CTR predictions for items that are not warm (that is, $|\mathcal{Y}_m^+|= 0$ and $|\mathcal{Z}_m^+|\geq 0$), with special attention on cold start items. The idea is to learn the correlation between cold start items and those easy-to-learn warm start items. To achieve this, we encode item correlations through their impression data with a pre-embedding model on warm start items. Before training the CTR model, for each item (including warm start and cold start items) we collect its user impressions to evaluate its similarity to a few pre-selected ``seed items". These similarity scores are transformed into a vector to initialize the item embedding for succeeding CTR training. We summarize our training pipeline in Figure~\ref{fig:embedding_init}. The main technical challenge is to learn a similarity score that reflects the distance between items' impression data distributions, which will be discussed in the next section.

% The key idea is to train an anomaly detection (AD) model with impression data on warm start items. The output of an AD model is a score representing familiarity between a user and an item. Loosely speaking, familiarity scores are higher when an item has been viewed by many similar users. Before training the CTR model, for each item (including warm and cold items), we collect its user impressions and evaluate the familiarity score between those users and a few pre-selected ``seed items". Those scores are transformed into a vector to initialize the item embedding for succeeding CTR training. We summarize our training pipeline in Figure~\ref{fig:embedding_init}.

Compared to existing methods for cold start initialization such as WMF~\cite{hu2008collaborative} and DropoutNet~\cite{volkovs2017dropoutnet}, our method has the following advantages. First, it only requires forward passes to initialize cold item embeddings. Second, it does not require context information when impression data is present. Third, it works consistently for both warm start and cold start items for any CTR model so one can seamlessly integrate it to existing systems.

% The main technical challenge is to learn a familiarity score that clearly differentiate among users conditioning on each item. When treating each item as a single task, we need to collaboratively learn those tasks given the potentially huge number of items. To this end, we propose collaborative anomaly detection (CAD) that jointly learn the likelihood ratio as the familiarity score for all tasks. CAD is a scalable method that generalize to thousands of tasks, which is intractable for existing single-task AD methods.


==> tables/cifar10_embedding_results.tex <==
\begin{table*}[t]%\footnotesize
  \caption{%\footnotesize
    %   Cross-domain matching results in terms of Recall@$K$ (R@K). The results in the first section is on Flickr30K. The results in the second section is on MSCOCO.
    Collaborative anomaly detection results in terms of AUC\;(\(\times\)100).  Label embedding uses prior knowledge (ground truth label) so it has a natural advantage comparing with other methods (Note that the first method ``label embedding'' uses extra knowledge and is marked with *. The best results without extra knowledge are shown in bold.).
    %*Means extra knowledge (ground truth category) is used in training.
  }\label{table:toy_result}
  \begin{center}
    \begin{small}
      \begin{sc}
        % \vspace{-3mm}
        % \begin{tabular}{lccccccc}
        \begin{tabular}{ccccccc}
          \toprule
          \multicolumn{1}{c|}{}                       & \multicolumn{2}{c|}{MNIST} & \multicolumn{4}{c}{CIFAR10}                                                                            \\
          \multicolumn{1}{c|}{K (\#tasks)}            & 4 (210)                    & \multicolumn{1}{c|}{5 (252)}        & 2 (45)         & 3 (120)        & 4 (210)        & 5 (252)       \\
          \midrule
          \multicolumn{1}{c|}{Label Embedding*}       & 99.88                      & \multicolumn{1}{c|}{99.67}          & 96.50           & 95.13          & 94.21          & 91.90          \\
          \multicolumn{1}{c|}{Pseudo Label Embedding} & 97.88                      & \multicolumn{1}{c|}{98.67}          & 96.00           & 94.13          & 92.21          & 85.90          \\
          %\multicolumn{1}{c|}{Multiple Output Heads}  & \textbf{99.94}             & \multicolumn{1}{c|}{99.76}          & \textbf{96.67} & \textbf{95.08} & \textbf{93.54} & 89.38         \\
          \multicolumn{1}{c|}{Random Initialization}  & 97.02                      & \multicolumn{1}{c|}{86.80}          & 95.97          & 93.07          & 87.13          & 78.96         \\
          \multicolumn{1}{c|}{Dual Embedding (dim = 10)}        & 98.88                      & \multicolumn{1}{c|}{99.67}          & 96.20           & 94.61          & 92.11          & 90.30          \\
          \multicolumn{1}{c|}{Dual Embedding (dim = 64)}        & \textbf{99.93}             & \multicolumn{1}{c|}{\textbf{99.90}} & \textbf{96.43}          & \textbf{95.06} & \textbf{93.45}          & \textbf{91.40} \\
          % \multicolumn{1}{l}{}                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
          \bottomrule
        \end{tabular}
      \end{sc}
    \end{small}
    % \vspace{-5mm}
  \end{center}
\end{table*}


==> tables/cifar_gen.tex <==
% \begin{wraptable}[12]{r!}{0.5\textwidth}
\begin{table}[t]
    \caption{Generalization performance of anomaly detection on CIFAR10 in terms of AUC\;(\(\times\)100). Rows index tasks for training and columns index tasks for testing.}\label{table:cifar_gen}
    \begin{center}
        \begin{small}
            \begin{sc}
                \begin{tabular}{c|cccc}
                    \toprule
                    train \(k\)\textbackslash{}test \(k\) & 2(45) & 3(120) & 4(210) & 5(252) \\
                    \midrule
                    % 2                                     & 97.02 & 89.11  & 79.33  & 73.11  \\
                    2                                     & -- & 89.11  & 79.33  & 73.11  \\
                    % 3                                     & 95.80 & 92.79  & 86.62  & 80.53  \\
                    3                                     & 95.80 & --  & 86.62  & 80.53  \\
                    % 4                                     & 95.26 & 93.94  & 90.98  & 86.52  \\
                    4                                     & 95.26 & 93.94  & --  & 86.52  \\
                    % 5                                     & 91.96 & 91.61  & 91.08  & 90.15  \\
                    5                                     & 91.96 & 91.61  & 91.08  & --  \\

                    \bottomrule
                \end{tabular}
            \end{sc}
        \end{small}
    \end{center}
\end{table}\vspace{-10pt}

% \end{wraptable}


==> tables/dataset_settings.tex <==
% \begin{table*}[]
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{3}{*}{\diagbox[width=3.4cm, height=1.2cm]{\vspace{1pt}Method}{Task}}   & \multicolumn{4}{c|}{Train}                                        & \multicolumn{4}{c|}{Test (100$\times$ Recall@10 )}                        \\ \cline{2-9} 
%                     & \multicolumn{2}{c|}{warm items} & \multicolumn{2}{c|}{cold items} & \multicolumn{2}{c|}{warm items} & \multicolumn{2}{c|}{cold items} \\ \cline{2-9} 
%                     & click       & impression       & click       & impression       & click        & impression      & click       & impression       \\ \hline
% full explicit only  & $\checkmark$   &                & $\checkmark$   &                & 7.71            &       -       & 8.11           &       -        \\ \hline
% full implicit only  &                & $\checkmark$   &                & $\checkmark$   &    -            & 9.49          &      -         & 9.14           \\ \hline
% full joint training & $\checkmark$   & $\checkmark$   & $\checkmark$   & $\checkmark$   & 11.94           &               & 11.60          &                \\ \hline
% warm joint training & $\checkmark$   & $\checkmark$   &                & $\checkmark$   & 13.61           &               & 10.87          &                \\ \hline
% ours cold start      & $\checkmark$   & $\checkmark$   &                &      \ding{108}          & 12.02                &               &   11.40        &                \\ \hline
% \end{tabular}
% \caption{This table describes four different training settings. The $\checkmark$ represents the data is used in the training process with back propagation. \ding{108} means the data is used with forward pass only. The experiments is completed on Movielens-1M}
% \end{table*}
% \usepackage{multirow}
% \usepackage{hhline}
% \usepackage{colortbl}
% \begin{minipage}{0.49\textwidth}
\begin{table}[t]
\vspace{-5pt}
\caption{Experimental setting and their corresponding recall@10 score on Movielens-1M. Warm and cold represents two non interacted item sets.  The checkmark means the corresponding data is used during the training with propagation. \ding{108} means the data is used with forward pass only. IMP. is the short form of impression. }
\begin{minipage}{0.49\textwidth}
\begin{center}
\begin{small}
\begin{sc}
\scalebox{0.75}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{c|cc|cc|cc|cc}
\toprule
\multirow{3}{*}{} & \multicolumn{4}{c|}{Train}                                & \multicolumn{4}{c}{Test (100$\times$Recall@10 )}    \\ \cmidrule{2-9} 
                  & \multicolumn{2}{c}{warm}   & \multicolumn{2}{c|}{cold}   & \multicolumn{2}{c}{warm} & \multicolumn{2}{c}{cold} \\ \cmidrule{2-9} 
                  & click        & imp.         & click        & imp.         & click        & imp.       & click        & imp.       \\ \midrule
                  
click only        & $\checkmark$ &              & $\checkmark$ &              & 8.10        & -          & 8.31         & -          \\
imp. only         &              & $\checkmark$ &              & $\checkmark$ & -            & 9.18       & -            & 8.55       \\
joint             & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & 9.88         & 9.07       & 9.84         & 9.68       \\
warm joint        & $\checkmark$ & $\checkmark$ &              & $\checkmark$ & 10.04        & 8.91       & 5.87         & 9.12       \\ \midrule
ours              & $\checkmark$ & $\checkmark$ &              &         \ding{108}    & 8.33         & -          & 7.81         & -          \\ \midrule

\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\end{minipage}
% \hspace{15pt}
\label{table:settings}
\end{table}
% \end{minipage}

==> tables/dataset_stats.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]\vspace{-10pt}
\label{table:stats}
\caption{Datasets statistics after prepossessing.}
\begin{minipage}{0.49\textwidth}
\begin{center}
\begin{small}
\begin{sc}
\scalebox{0.75}{
\begin{tabular}{@{}cc|cc|cc@{}}
\toprule
                                           &            & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Movielens-1M\\ (user: 6040)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Book-Crossing\\ (user: 15798)\end{tabular}} \\ \cmidrule(l){3-6} 
                                           &            & items                                  & interactions                                 & items                                    & interactions                                    \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{warm}} & impression & 2.86k                                  & 800k                                         & 30.4k                                    & 448k                                            \\
\multicolumn{1}{c|}{}                      & click      & 2.77k                                  & 460k                                         & 24.1k                                    & 11.8k                                           \\
\multicolumn{1}{c|}{\multirow{2}{*}{cold}} & impression & 0.717k                                 & 200k                                         & 7.62k                                    & 107k                                            \\
\multicolumn{1}{c|}{}                      & click      & 0.671k                                 & 115k                                         & 6k                                       & 28.4k                                           \\ \bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\end{minipage}
% \hspace{15pt}
\end{table}

==> tables/mnist_auc_results.tex <==
\begin{table}[t]
\caption{Testing AUC\;(\(\times\)100) on CIFAR10 with $k=1,2,3,4$. The number in the brackets represents the total number of tasks. (Left) Conditional (collaborative) learning. (Right) Separate learning. }\label{table:cifar10}
\begin{minipage}{0.49\textwidth}
\begin{center}
\begin{small}
\begin{sc}
\scalebox{0.8}{
\begin{tabular}{c|cccc}
\toprule
Method~\textbackslash{}~k & 1(10) & 2(45) & 3(120) & 4(210) \\
\midrule
GMM & 88.2 & 73.9 & 68.1 & 64.1 \\
MAF & 86.1  & 74 & 62.6 & 58.9\\
GLOW & 96.7 & 58.9 &  & \\
LRatio & 99.9 & 99.9 & 99.9 & 99.9\\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{center}
\begin{small}
\begin{sc}
\scalebox{0.8}{
\begin{tabular}{c|cccc}
\toprule
Method~\textbackslash{}~k & 1(10) & 2(45) & 3(120) & 4(210) \\
\midrule
GMM &  &  &71.2 & \\
MAF &  &  & 76.6 & 74.11 \\
GLOW &  & 86 &  & 80.1 \\
LRatio &  &  &  & \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\end{minipage}
\end{table}

==> tables/performance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\caption{Results on datasets without content information.}
\vspace{5pt}
\begin{minipage}{\textwidth}
\begin{center}
% \begin{small}
\begin{sc}
\scalebox{0.9}{
\begin{tabular}{@{}c|ccccc|ccccc@{}}
\toprule
Dataset               & \multicolumn{5}{c|}{Movielens-1M}                                                & \multicolumn{5}{c}{Book Crossing}                                               \\ \midrule
metrics(@10)          & F1            & precision      & recall        & hit            & ndcg           & F1           & precision     & recall         & hit            & ndcg           \\ \midrule
random initialization & 1.52          & 3.25           & 2.76          & 24.61          & 14.10          & 1.33         & 0.80          & 5.87           & 7.92           & 6.3            \\
click only*           & \textit{7.09} & \textit{18.19} & \textit{8.31} & \textit{60.63} & \textit{41.24} & \textit{2.5} & \textit{1.60} & \textit{10.15} & \textit{14.73} & \textit{10.40} \\
warm joint**          & 4.72          & 8.65           & 5.87          & 52.91          & 30.04          &              &               &                &                &                \\
imp. label (i-w)      & 2.43          & 5.42           & 3.31          & 35.43          & 21.51          &              &               &                &                &                \\
imp. label (u-w)      & 4.93          & 8.55           & 7.24          & 51.97          & 30.56          & 1.99         & 1.23          & 8.36           & 11.89          & 7.80           \\
WMF embedding         & 4.74          & 8.43           & 6.56          & 51.97          & 31.38          &              &               &                &                &                \\
Log Ratio (ours)      & \textbf{5.23} & \textbf{9.09}  & \textbf{7.81} & \textbf{54.33} & \textbf{31.82} & 2.09         & 1.3           & 8.82           & 12.53          & 8.13           \\ \bottomrule
\end{tabular}
}
\end{sc}
% \end{small}
\end{center}
\end{minipage}
% \hspace{15pt}\caption{1. Results on the click testing set of all the cold items. 2. Pretrain on the impression data. 3. No content information used. }
\label{table:no_content}
\end{table*}

==> tables/related_mtl.tex <==
\begin{table}[t]
    \caption{Description of our methods is bad. Consider a better way later.}\label{table:related_ml}
    \begin{tabular}{l|l}
        (a) Task Embedding        & \(g(f(\xv_t, \ev_t))\)              \\
        (b) Multiple Output Heads & \(g_t(f(\xv_t))\)                   \\
        (c) Variable Embeddings   & \(g(\sum_i f(x_i,\ev_i), \ev_j)  \) \\
        (d) Dual Embeddings       &                                     \\
        % (d) Dual Embeddings       & \(f_2((\sum_i \sum_j g_j(f_1(\xv_i))), \xv_i)\)
    \end{tabular}
\end{table}


==> tables/toy_results.tex <==
\begin{table*}[t]%\footnotesize
  \caption{%\footnotesize
    %   Cross-domain matching results in terms of Recall@$K$ (R@K). The results in the first section is on Flickr30K. The results in the second section is on MSCOCO.
    Collaborative anomaly detection results in terms of AUC\;(\(\times\)100).  Label embedding uses prior knowledge (ground truth label) so it has a natural advantage comparing with other methods (Note that the first method ``label embedding'' uses extra knowledge and is marked with *. The best results without extra knowledge are shown in bold.).
    %*Means extra knowledge (ground truth category) is used in training.
  }\label{table:toy_result}
  \begin{center}
    \begin{small}
      \begin{sc}
        % \vspace{-3mm}
        % \begin{tabular}{lccccccc}
        \begin{tabular}{ccccccc}
          \toprule
          \multicolumn{1}{c|}{}                       & \multicolumn{2}{c|}{MNIST} & \multicolumn{4}{c}{CIFAR10}                                                                            \\
          \multicolumn{1}{c|}{K (\#tasks)}            & 4 (210)                    & \multicolumn{1}{c|}{5 (252)}        & 2 (45)         & 3 (120)        & 4 (210)        & 5 (252)       \\
          \midrule
          \multicolumn{1}{c|}{Label Embedding*}       & 99.88                      & \multicolumn{1}{c|}{99.67}          & 96.50           & 95.13          & 94.21          & 91.90          \\
          \multicolumn{1}{c|}{Pseudo Label Embedding} & 97.88                      & \multicolumn{1}{c|}{98.67}          & 96.00           & 94.13          & 92.21          & 85.90          \\
          %\multicolumn{1}{c|}{Multiple Output Heads}  & \textbf{99.94}             & \multicolumn{1}{c|}{99.76}          & \textbf{96.67} & \textbf{95.08} & \textbf{93.54} & 89.38         \\
          \multicolumn{1}{c|}{Random Initialization}  & 97.02                      & \multicolumn{1}{c|}{86.80}          & 95.97          & 93.07          & 87.13          & 78.96         \\
          \multicolumn{1}{c|}{Dual Embedding (dim = 10)}        & 98.88                      & \multicolumn{1}{c|}{99.67}          & 96.20           & 94.61          & 92.11          & 90.30          \\
          \multicolumn{1}{c|}{Dual Embedding (dim = 64)}        & \textbf{99.93}             & \multicolumn{1}{c|}{\textbf{99.90}} & \textbf{96.43}          & \textbf{95.06} & \textbf{93.45}          & \textbf{91.40} \\
          % \multicolumn{1}{l}{}                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
          \bottomrule
        \end{tabular}
      \end{sc}
    \end{small}
    % \vspace{-5mm}
  \end{center}
\end{table*}

